Q-Mixing Network for Multi-Agent Pathfinding in Partially Observable Grid Environments

In this paper, we consider the problem of multi-agent navigation in partially observable grid environments. This problem is challenging for centralized planning approaches as they, typically, rely on the full knowledge of the environment. We suggest utilizing the reinforcement learning approach when the agents, first, learn the policies that map observations to actions and then follow these policies to reach their goals. To tackle the challenge associated with learning cooperative behavior, i.e. in many cases agents need to yield to each other to accomplish a mission, we use a mixing Q-network that complements learning individual policies. In the experimental evaluation, we show that such approach leads to plausible results and scales well to large number of agents.

==> ru/01-abstract.tex <==
\begin{abstract}
В настоящей работе рассматривается задача обучения генерации целенаправленного поведения группой интеллектуальных агентов, перемещающихся в клеточной среде с ограниченной областью видимости. В данной постановке задачи оказываются плохо применимыми классические методы многоагентного поиска пути, т.к. они, в основном, исходят из предположения о доступности полной информации о среде или возможности полного сохранения всех ранее доступных прецедентов планирования. В данной работе предложена адаптация смешивающей Q-сети, реализующей многоагентное обучение с подкреплением, для планирования перемещения в клеточной среде. Была создана экспериментальная программная реализация данной среды для проверки работоспособности предложенного подхода, проведено сравнение для различных конфигураций задачи с одноагентными методами обучения с подкреплением.
% и методами семейства A* с неограниченной памятью.
\keywords{Многоагентное планирование пути \and Обучение с подкреплением \and Смешивающая Q-сеть \and Клеточная среда}
%\keywords{Multiagent Path Finding \and Reinforcement Learning \andMixing Q-network \and Grid Environment}
\end{abstract}

==> ru/02-introduction.tex <==
\section{Введение}
Планирование перемещения группы интеллектуальных агентов обычно рассматривается как отдельное направление планирования поведения и для решения этой задачи применяются методы, которые условно можно разделить на две группы: централизованные и децентрализованные. Методы первой группы опираются на предположение о существовании единого центра управления агентами, которому доступна полная информация о состояниях и перемещениях агентов в любой момент времени. В большинстве случаев в основе таких методов лежит либо сведение задачи многоагентного планирования к другим известным задачам, таким как, например, задача о выполнимости булевых формул (SAT-задачи)~\cite{surynek2016efficient}, либо использование методов и инструментов эвристического поиска для отыскания решения. Среди последних наиболее активно развиваются в последнее время алгоритмы семейства CBS (Conflict based search)~\cite{sharon2015conflict}. Классический алгоритм CBS гарантирует оптимальность отыскиваемых решений. Существует множество его улучшений, сохраняющих такую гарантию и на практике существенно увеличивающих вычислительную эффективность алгоритма -- ICBS~\cite{boyarski2015icbs}, CBSH~\cite{felner2018adding}. Также известны адаптации CBS для учета кинематических ограничений, получения ограниченно-субоптимальных решений~\cite{barer2014suboptimal}. Другим широко-распространенными подходом к централизованному планирования является приоритизированное планирование~\cite{yakovlev2019prioritized}, которое, однако, не гарантирует решения задачи в общем случае, но при этом предоставляют такую гарантию, когда выполняется определенный набор условий~\cite{cap2015a}. На практике такие условия соблюдаются, например, в складской робототехнике, поэтому приоритизированные методы активно в ней применяются.


Вторая группа методов предполагает децентрализованную реализацию, в которой агенты более автономны и находятся в условиях неполной информации, получая только ограниченный доступ к данным о своих перемещениях и перемещениях других агентов. Частным случаем такой постановки задачи является вариант частично наблюдаемой среды, в которой агент может наблюдать только некоторую окрестность среды вокруг себя: препятствия, свою целевую область, других агентов и их цели. Данная постановка задачи интересна тем, что она полнее реализует реальные условия при навигации робототехнических платформ и позволяет предложить методы по учету действий других агентов в условиях неполной или неточной информации (отсутствие сигналов GPS, зашумленные, неточные сенсоры и т.д.). В данной работе задача рассматривается именно при условии частичной наблюдаемости.

Одними из наиболее широко-распространенных методов решения задачи много-агентной навигации в такой постановке являются алгоритмы семейства ORCA~\cite{van2011reciprocal}. В основу этих алгоритмов заложен принцип выбора текущей скорости из так называемого пространства безопасных скоростей. При выполнении определенных условий ORCA гарантирует отсутствие столкновений между агентами, однако гарантий на достижение цели не предоставляется. На практике, при навигации в ограниченном пространстве (помещение с узкими коридорами, проходами и пр.) агенты часто попадают в ситуацию ``мертвого замка'', когда агенты снижают свою скорость до нуля, чтобы избежать столкновения друг с другом, и перестают двигаться к целям. Важно также отметить, что в своей работе алгоритмы семейства ORCA опираются на знание векторов скоростей других агентов. В представленной работе такого предположения не делается и предлагается применять обучаемые методы, в частности -- методы обучения с подкреплением, для решения рассматриваемой проблемы.

Использование алгоритмов обучения с подкреплением для задачи поиска пути в частично наблюдаемых средах предлагалось и ранее. Так, в статье~\cite{panov2018grid} авторы рассматривают одногоагентный случай частично наблюдаемой среды и применяют алгоритм глубокой Q-сети ~\cite{mnih2015human} (DQN) для его решения.  

В статье~\cite{sartoretti2019primal} рассматривается многоагентный случай постановки этой задачи. Нейросетевой аппроксиматор подбирает параметры, используя один из классических алгоритмов глубокого обучения с подкреплением. Однако полноценная работа алгоритма возможна только при пополнении опыта агента экспертными данными, выбранными на основе оптимального пути, который строится классическим планировщиком. Подход не использует максимизацию общей функции полезности, а пытается решить проблему многоагентного взаимодействия введением различных эвристик: дополнительная функция потерь за блокирование других агентов; функция вознаграждения, которая учитывает столкновение агентов; кодирование целей других агентов в наблюдении. 

В настоящей работе мы предлагаем решать поставленную задачу с помощью обучаемых методов генерации поведения на основе обучения с подкреплением. В качестве методологической базы мы предлагаем использовать смешивающую Q-сеть, которая реализует принцип монотонного улучшения общей оценки полезности текущего состояния на основе текущих оценок полезности состояния отдельных агентов. Обучение механизма смешивания на основе параметризованного аппроксиматора позволяет автоматически формировать правила разрешения конфликтных ситуаций, возникающих при построении и прохождении пересекающихся участков пути двумя и более агентами. Также мы предлагаем реализацию гибкой и эффективной экспериментальной среды с планированием траекторий для группы агентов с ограниченными областями видимости. Конфигурируемость и возможность реализации различных поведенческих сценариев за счет изменения функции вознаграждения позволяет провести сравнение предложенного метода как с классическими методами многоагентного планирования траекторий, так и с методами обучения с подкреплением, рассчитанными на обучение одного агента.

==> ru/03-task.tex <==
\section{Постановка задачи}

Задачу поиска пути несколькими агентами в частично-наблюдаемой среде будем сводить к задаче одногоагентного обучения с использованием подкрепляющего сигнала с некоторыми ограничениями, которая накладываются на процесс обучения агентов. Процесс взаимодействия агента и среды будет моделироваться марковским процессом принятия решений. Результатом обучения будет служить стратегия, отображающая пространство наблюдений агента в пространство действий. Данная функция будет генерировать поведение агента и будет учитывать возможные конфликтные ситуации при перемещении нескольких агентов.

Марковский процесс принятия решений описывается как четверка $<S, A, P, r, \gamma>$. $s \in S$ описывает состояние среды. Каждый шаг в среде агент выполняет действие $a \in A$ и получает за данное действие награду по функции вознаграждения $r(s, a): S \times A \rightarrow {\mathbb R}$. Данное действие инициирует переход в среде $P(s'|s, a): S \times A \times S \rightarrow [0, 1]$. Агент использует полученную из среды информацию для автоматического формирования функции стратегии $\pi(a|s): A \times S \rightarrow [0, 1]$. Во многих случаях эффективнее формировать функцию полезности  $Q(a_t, s_t) = r(s_t, a_t) + \mathbb E ( \sum_{i=1}^\infty \gamma^i r(s_{t+i}, a_{t+i} ) )$, где $\gamma$ -- фактор дисконтирования.

Частично наблюдаемый марковский процесс принятия решений отличается от стандартной постановки тем, что вводится отдельный набор возможных наблюдений агента $O$, в общем случае не совпадающий с множеством состояний $S$: $<S, O, A, P, r, \gamma>$. В данном случае агент получает от среды не ее состояние, а некоторое наблюдение $o$. Соответственно стратегия и функция полезности строятся на основе наблюдения: $\pi(a|o): A \times O \rightarrow [0, 1]$, $Q(a_t, o_t) = r(s_t, a_t) + \mathbb E ( \sum_{i=1}^\infty \gamma^i r(s_{t+i}, a_{t+i} ) )$.

В задаче нахождения пути для множества агентов среда представляет из себя граф регулярной структуры (клеточное поле), в котором некоторое подмножество узлов отвечают за препятствия, другая подмножество -- доступные агентам положения, в т.ч. и цели для агентов. Задачей агентов является построение оптимального (кратчайшего) путь до своей цели. В данной задаче состояние $s\in S$ описывает расположение препятствий, агентов и целей агентов. Наблюдение $o\in O$ описывает информацию о расположении препятствий, агентов и целей в радиусе вокруг конкретного агента. Агенты могут совершать действия для перемещения по осям $X$ и $Y$ по клеточному полю.

==> ru/04-method.tex <==
\section{Метод}
% \subsection{Аппроксимационное Q-обучение}

%\todo[Дать простое описание DQN. Мы учимся оценивать полезности, а потом зная их можем максимизировать награду. Почему это работает плохо для двух агентов. Идея Q-mix добавляем максимизацию и общей функции полезности для агентов. Пример раскадровки анимации, где агенты максимизирующей только свою функцию полезности не доходят до целей. И пример, где доходят.]

В настоящей работе мы предлагаем оригинальную архитектуру принятия решений и обучения агента на основе смешивающей Q-сети, использующей глубокие нейросетевые аппроксиматоры для параметризации функции полезности по аналогии с глубоким Q-обучением (DQN).

В глубоком Q-обучении подбираются параметры нейросетевого аппроксиматора для функции полезности $Q(a, s| \theta )$. Обновление параметров  происходит для мини-выборок (батчей) опытных данных агента, состоящих из четверок $<s, a, r, s'>$, где $s'$ -- это состояние, в которое агент перешел после выполнения действия $a$ в состоянии $s$. Функция потерь для аппроксиматора выглядит следующим образом:

\[ L=\sum_{i=1}^{b} [((r^i+\gamma max_{a^{i+1}}Q(s^{i+1}, a^{i+1}|\theta)) - Q(s^i, a^i |\theta))^2], \] 
где b - размер батча.

При переходе к многоагентному обучению с подкреплением одним из вариантов реализации процесса обучения является независимое исполнение. В данном подходе агенты оптимизируют собственные $Q$ функции для действий одного агента. От DQN данный подход отличается процессом обновленяи параметров аппроксиматора, когда агенты используют информацию полученную от других агентов. По сути агенты проводят декомпозицию функции полезности (VDN)~\cite{Sunehag2017} и ставят себе целью максимизацию общей Q-функции $Q_{tot} (\tau, u)$, которая является суммой Q-функций каждого отдельного агента $Q^i (a^i, s^i | \theta^i)$.

Алгоритм смешивающей Q-сети (QMIX)~\cite{Rashid2018} работает аналогично VDN. Однако в данном случае для вычисления $Q_{tot}$ используется новая параметризованная функция от всех Q-значений агентов. Точнее, $Q_{tot}$ вычисляется так, чтобы выполнялось условие, что $Q_{tot}$ монотонно возрастает с ростом $Q^i$:

\[ \frac{\delta Q_{tot} }{\delta Q^i} \geq 0 \; \forall i \; 1 \leq i \leq num \, agents \]

$Q_{tot}$ параметризуется с помощью так называемой смешивающей нейронной Q-сети. Веса для данной сети генерируются с помощью гиперсетей ~\cite{Ha2016}. Каждая из гиперсетей состоит из единственного полносвязного слоя с модульной функцией активации, которая гарантирует неотрицательные значения в весах смешивающей сети. Отступы для смешивающей сети генерируются аналогично, однако они могут быть отрицательными. Последний отступ смешивающей сети генерируется с помощью двухслойной гиперсети с активацией ReLU. 

К особенностям работы смешивающей сети относится и то, что состояние или наблюдение агента не подается в сеть, так как $Q_{tot}$ не обязан монотонно возрастать при изменении параметров состояния $s$. Индивидуальные функции $Q^i$ получают на вход только наблюдение, которое может лишь частично отражать общее состояние среды. Так как состояние может содержать в себе полезную информацию для обучения его необходимо использовать и при вычислении $Q_{tot}$, потому состояние $s$ подается на вход гиперсети. Таким образом, $Q_{tot}$ опосредованно зависит от состояния среды и объединяет в себе все Q-функции агентов. Архитектура смешивающей сети представлена на рисунке~\ref{fig:qmix-scheme}.

Функция потерь для смешивающей сети выглядит аналогично функции ошибок для DQN:

\[ \sum_{i=1}^{b} [({y^i_{tot}} - Q_{tot}(\tau^i, u^i, s^i|\theta))^2] \] 

\[ y_{tot}=r+\gamma max_{t'}Q_{tot}(\tau', u', s'|\theta^-). \]
Здесь $b$ -- это размер батча для обучения, $\tau'$ -- действие, которое будет выполнено на следующем шаге после получения вознаграждения $r$, $u'$ --  наблюдение, полученное на следующем шаге, $s'$ -- состояние, полученное на следующем шаге. $\theta^-$ это параметры копии смешивающей Q-сети, создаваемой для стабилизации целевой переменной.

\begin{figure}
\centerline{\includegraphics[width=0.8\linewidth]{figures/minxing-network-normal.png}}
    \caption{a) Архитектура смешивающей сети. $W_1$, $W_2$, $B_1$, $B_2$ -- веса смешивающей сети; $Q_1$, $Q_2$ ... $Q_n$ - Q-значения агентов; $s$ -- состояние среды; $Q_{tot}$ - общее Q значение; b) Архитектура гиперсети для генерации матрицы весов для смешивающей сети. Гиперсеть состоит из одного полносвязного слоя и модульной функции активации. c) Архитектура гиперсети для генерации отступов для смешивающей сети. Гиперсеть состоит из одного полносвязного слоя.}
\label{fig:qmix-scheme}
\end{figure}


==> ru/05-environment.tex <==
\section{Экспериментальная среда для многоагентного планирования}
Среда представляет собой клеточное поле с расположенными на нём агентами, их целями и препятствиями. Каждому агенту необходимо добраться до своей цели, избегая препятствий и других агентов. Пример среды, показывающей частичную наблюдаемость для одного агента представлен на рисунке~\ref{fig:env-example}. Также на этом рисунке показан пример среды для нескольких агентов.

% \begin{figure}
% \centerline{\includegraphics[height=5cm]{figures/environment2.png}}

% \label{fig:env-example}
% \end{figure}

\begin{figure*}[ht]
    \centering
    \subfigure{\includegraphics[width=0.42\linewidth]{figures/with-projection-0473-crop.pdf}}
    \hspace{0.1\linewidth}
    \subfigure{\includegraphics[width=0.42\linewidth]{figures/10agents0751.pdf}}

    \caption{На левом рисунке показан пример частичной наблюдаемости для среды с одним агентом: серые вершины -- свободные клетки, по ребрам которых агент может перемещаться; заполненный красный круг показывает положение одного из агентов; вершина с красной обводкой -- цель этого агента, вершина с красной границей -- проекция цели агента. Область, которую агент не видит показана прозрачной.
    На правом рисунке показан пример среды для 8 агентов, проекции целей агентов и частичная наблюдаемость, не показаны из соображений наглядности.}
    \label{fig:env-example}
\end{figure*}

Входными параметрами при генерации среды являются: 
\begin{itemize}
    \item размеры поля $E_{size} \geq 2$,
    \item плотность препятствий $E_{density}\in[0, 1)$,
    \item количество агентов в среде $E_{agents} \geq 1$,
    \item радиус обзора: агентам доступны $1 \leq R \leq E_{size}$ клеток в каждую сторону,
    \item максимальное количество шагов, которое каждый из агентов может сделать до завершения эпизода $E_{horizon} \geq 1$,
    \item дистанция до цели каждого из агентов $E_{dist}$ (является необязательным параметром, если не задан, то дистанция до цели для каждого из агентов определяется случайно). 
\end{itemize}

Матрица препятствий заполняется случайным образом по параметрам $E_{size}$ и $E_{density}$. Положения агентов и их цели также определяются случайным образом, но с гарантией достижимости.

Пространство наблюдений $O$ каждого из агентов представляет собой многомерную матрицу: $O: 4 \times \big(2\times R + 1\big) \times \big(2\times R + 1 \big)$, которая включает в себя следующие 4 матрицы. \textit{Матрица препятствий}: $1$ кодирует препятствие, а $0$ его отсутствие. Если какая-то клетка области обзора агента выходит за рамки среды, то она кодируется $1$. \textit{Матрица положения агентов}: $1$ кодирует другого агента в ячейке, а $0$ его отсутствие. В центре хранится значение обратно пропорциональное расстоянию до цели агента. \textit{Матрица целей других агентов}: $1$ если цель какого-то агента находится в клетке, $0$ -- иначе. \textit{Матрица цели агента}: если цель в области наблюдения, то в клетке, где она находится будет $1$, а во всех остальных клетках будет $0$. Если же цель не попадает в область видимости, то она проецируются на ближайшую клетку области наблюдения. В качестве клетки для проекции выбирается клетка, на границе области видимости, которая либо имеет такую же координату по одной из осей, как и у целевой клетки, либо если таких клеток нет, то выбирается ближайшая угловая клетка области видимости. Пример пространства наблюдения агента представлен на рисунке~\ref{fig:observation-space}.

\begin{figure}
\centerline{\includegraphics[width=\textwidth]{figures/observtion_v2.png}}
\caption{Пример матрицы наблюдения для фиолетового агента. Во всех клетках наблюдения 1 означает, что в данной клетке есть объект(препятствие, агент или цель) и 0 иначе. a) Состояние среды. Рамкой выделен агент, для которого показано наблюдение; b) Карта препятствий. Центральная клетка соответствует положению агента, в данной карте объектами являются препятствия; c) Карта агентов, в данной карте объектами являются агенты; d) Карта целей других агентов, в данной карте объектами являются цели других агентов; e) Карта собственной цели, в данной карте объектом является собственная цель агента.}
\label{fig:observation-space}
\end{figure}

Каждому агенту доступны 5 действий: остаться на месте и переместиться вертикально (вверх или вниз) или горизонтально (вправо или влево). Агент может переместиться в любую свободную клетку, не занятую препятствием или другим агентом. Если агент перемещается в клетку с собственной целью, то он удаляется с карты, эпизод для него завершен.

Агенты получают вознаграждение $0.5$, если он идет по одному из оптимальных маршрутов к своей цели, $-1$, если агент увеличил свое расстояние до цели и $-0.5$, если агент остался на месте.


==> ru/06-experiments.tex <==
\section{Эксперименты}

В данном разделе приведены результаты сравнения QMIX с алгоритмом по актуальному опыту -- методом оптимизации ближайшей стратегии (PPO)~\cite{schulman2017proximal}. PPO был выбран, т.к. он показал лучшие результаты в многоагентной постановке по сравнению с другими современными алгоритмами обучения с подкреплением. Также, этот алгоритм существенно превзошел остальные алгоритмы, включая QMIX, в одноагентном случае.

Обучение различных вариантов алгоритмов происходило на средах размером $ E_{size} = 15 \times15 $, со следующими параметрами: $ E_{density} = 0.3 $, $ E_{agents} = 2 $, $ R = 5 $, $ E_{horizon} = 30 $, $ E_{dist} = 8 $. В качестве основной архитектуры сети каждого из методов использовалась архитектура с двумя скрытыми слоями размером $ 64 $ нейрона. В качестве функции активации для QMIX использовалась функция ReLU, а для PPO использовалась функция $\tanh$ (гиперболический тангенс). Эксперименты были проведены в условиях ограниченного количества шагов взаимодействия со средой, на обучение было выделено 1.5 миллионов шагов. 

 

\begin{figure*}[ht]
    \centering
    \subfigure{\includegraphics[width=0.49\linewidth]{figures/15x15Random-crop.pdf}}
    \subfigure{\includegraphics[width=0.49\linewidth]{figures/15x15Hard-crop.pdf}}

    \caption{На графиках показаны отдельные кривые для разных размеров. В средах использовалось 2, 6, 16 агентов, для сред размером $8\times8$, $16\times16$, $32\times32$, соответственно. На левом графике показана зависимость успешных завершений среды в зависимости от шага обучения для алгоритма QMIX на случайных картах. На правом графике показана зависимость успешных завершений среды в зависимости от шага обучения для алгоритма QMIX на сложных выбранных картах. }
    \label{fig:qmix-training}
\end{figure*}

Результаты обучения алгоритма QMIX показаны на рисунке~\ref{fig:qmix-training}. Целью данной серии экспериментов было проверить способность QMIX агентов действовать субоптимально относительно жадной стратегии, но оптимально для кооперативной стратегии. Проверка алгоритма проводилась каждые 100 тысяч шагов на окружениях, которые алгоритм не видел во время обучения. Список этих окружений был фиксирован на протяжении всего обучения.  Также на этом рисунке представлены графики проверки алгоритма на сложных средах. Сложность окружений заключалась в том, что они были специально составлены так, чтобы часть агентов должна была сначала пропустить других, а только потом двигаться к своей цели. Пример трех сложных сред для размера карты $8\times8$ показан на рисунке~\ref{fig:hard70}.


\begin{figure*}[ht]
    \centering
    
    \subfigure{\includegraphics[width=0.29\linewidth]{figures/00028.pdf}}
    \hspace{0.03\linewidth}
    \subfigure{\includegraphics[width=0.29\linewidth]{figures/2agents-hard-0330.pdf}}
    \hspace{0.03\linewidth}
    \subfigure{\includegraphics[width=0.29\linewidth]{figures/2agents-hard-0473.pdf}}
    \caption{Примеры сложных сред размера $8\times8$, где агентам необходимо использовать кооперативную стратегию, чтобы дойти до цели. Во всех примерах оптимальные пути агентов до их целей пересекаются, и одному из них необходимо уступить путь другому. Прозрачными показаны вершины, которые не видны агентам.} 
    \label{fig:hard70}
\end{figure*}

После обучения каждого из алгоритмов было проведено финальное тестирования. Результаты этого тестирования показаны в таблице~\ref{table:eval-random} для случайных сред и в таблице~\ref{table:eval-hard} для сложных сред. По итогам обучения алгоритм QMIX оказался более успешен чем алгоритм PPO, что показывает важность использования общей функции полезности во время обучения.

\begin{table}[htp]
	  \caption{Сравнение на наборе из 200 сред (для каждого набора параметров)  со случайном сгенерированными препятствиями.
	  В последних двух столбцах показано среднее количество достижений агентами своих целей для PPO и QMIX соответственно. Результаты усреднены по 3 запускам каждого алгоритма в каждой среде. QMIX показывает лучшие результаты, благодаря использованию общей Q-функции $Q_{tot}$}
    \label{table:eval-random}
    \centering
    \begin{tabular}{p{0.12\textwidth}p{0.12\textwidth}p{0.05\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}}
        \toprule
            
         $E_{size}$ & $E_{agents}$ & $R$ & $E_{horizon}$ & $E_{dist}$& $E_{density}$ & PPO & QMIX\\
        \midrule
         $8\times8$ & 2 & 5 & 16 &  5 & 0.3 & 0.539 & \textbf{0.738} \\
         $16\times16$ & 6 &5 & 32 & 6 &  0.3 & 0.614 & \textbf{0.762} \\
        $32\times32$ & 16 & 5 & 64 & 8 & 0.5 & 0.562 & \textbf{0.659} \\
        \bottomrule
    \end{tabular}
    
\end{table}

\begin{table}[htp]
	  \caption{Сравнение на наборе из 70 сред (для каждого набора параметров) со сложными препятствиями. В последних двух столбцах показано среднее количество достижений агентами своих целей для PPO и QMIX, соответственно. Результаты усреднены по 10 запускам каждого алгоритма в каждой среде. QMIX также показывает результаты лучшие, чем алгоритм PPO.}
    \label{table:eval-hard}
    \centering
    \begin{tabular}{p{0.12\textwidth}p{0.12\textwidth}p{0.05\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}}
        \toprule
            
         $E_{size}$ & $E_{agents}$ & $R$ & $E_{horizon}$ & $E_{dist}$& $E_{density}$ & PPO & QMIX\\
        \midrule
         $8\times8$ & 2 & 5 & 16 &  5 & 0.3 & 0.454 & \textbf{0.614} \\
         $16\times16$ & 6 &5 & 32 & 6 &  0.3 & 0.541 & \textbf{0.66} \\
        $32\times32$ & 16 & 5 & 64 & 8 & 0.5 & 0.459 & \textbf{0.529} \\
        \bottomrule
    \end{tabular}
    
\end{table}






















% Для демонстрации работоспособности смешивающей Q-сети для задачи поиска пути несколькими агентами были проведены следующие эксперименты:
% \begin{enumerate}
%     \item эксперименты с одним агентом на случайных картах,
%     \item эксперименты с двумя агентами на случайных картах.
% \end{enumerate}

% Во всех экспериментах после каждых 50000 шагов в среде качество обучения агента проверялось на одних и тех же наборах карт размером $8\times 8$, $16\times 16$, $32\times 32$, $64\times 64$.

% \subsection{Эксперименты с одним агентом}
% Данные эксперименты были проведены с следующими параметрами:
% \begin{enumerate}
%     \item размер среды $6 \times 6$, расстояние до цели 5,
%     \item размер среды $10 \times  10$, расстояние до цели 5,
%     \item размер среды $15\times  15$, расстояние до цели 8,
%     \item размер среды $17\times  17$, расстояние до цели 10.
% \end{enumerate}

% Во всех экспериментах плотность препятствий была равна 0.3, радиус наблюдений -- 5, максимальное число шагов в эпизоде -- 50. Были протестированы алгоритмы смешивающей сети QMIX, PPO, D*Lite и A*Lite.

% \begin{figure}
% \centerline{\includegraphics[width=\textwidth]{figures/1agentreward.png}}
% \caption{График вознаграждений для одноагентного QMIX}
% \end{figure}

% \begin{figure}
% \centerline{\includegraphics[width=\textwidth]{figures/Finished1agent.png}}
% \caption{График процента успешных достижений цели для одноагентного QMIX}
% \end{figure}

% \subsection{Эксперименты с двумя агентами на фиксированной карте}
% Данные эксперименты были проведены с алгоритмом QMIX. Целью данной серии экспериментов было проверить способность агентов действовать субоптимально относительно жадной стратегии, но оптимально для кооперативной стратегии. Для прохождения сценария одному из агентов необходимо пропустить второго к их целям. Максимальное число шагов в эпизоде 1000.

% \subsection{Эксперименты с двумя агентами на случайной карте}
% Данные эксперименты были проведены с алгоритмом QMIX со следующими параметрами:
% \begin{enumerate}
%     \item размер среды $6 \times 6$, расстояние до цели 5,
%     \item размер среды $10 \times  10$, расстояние до цели 5,
%     \item размер среды $15\times  15$, расстояние до цели 8,
%     \item размер среды $17\times  17$, расстояние до цели 10.
% \end{enumerate}

% Во всех экспериментах плотность препятствий была равна -- 0.3, радиус наблюдений -- 5, максимальное число шагов в эпизоде -- 50. Для данных экспериментов алгоритм QMIX был запущен со следующей функцией вознаграждения: 1 если агент приближается к цели, -1 если удаляется и 0 иначе.

% \begin{figure}
% \centerline{\includegraphics[width=\textwidth]{figures/2agentsreward.png}}
% \caption{График вознаграждений для многоагентного QMIX}
% \end{figure}

% \begin{figure}
% \centerline{\includegraphics[width=\textwidth]{figures/Finished2agents.png}}
% \caption{График процента успешных достижений цели для многоагентного QMIX}
% \end{figure}

% \subsection{Эксперимент в сложных многоагентных средах}



==> ru/07-conclusion.tex <==
\section{Заключение}
В настоящей работы была рассмотрена задача многоагентного поиска пути при частичной наблюдаемости среды. Такая постановкой с неполной информацией приводит к невозможности применения классических методов многоагентного планирования траекторий, но позволяет применять алгоритмы обучения с подкреплением. Было предложено использовать для решения поставленной задачи смешивающую Q-сеть с нейросетевой аппроксимацией, которая подбирает параметры объединяющей функции полезности, комбинирующей функции полезности отдельных агентов. 
Была разработана экспериментальная программная среда для проведения экспериментов с обучаемыми алгоритмами. На данной среде была продемонстрирована работоспособность предложенного метода и его эффективность по сравнению с алгоритмами обучения с подкреплением по актуальному опыту (on-policy). Необходимо отметить, что сравнение проводилось в условиях ограничения  количества эпизодов взаимодействия агента со средой. В случае снятия такого ограничения эффективности метод по актуальному опыту может превзойти предложенный алгоритм смешивающей Q-сети, который являются методом обучения с отложенными опытом (off-policy). В дальнейших работах мы планируем совместить преимущества более качественного целенаправленного поведения, который генерирует метод по актульному опыту, и возможность учета действий другого агента при разрешении локальных конфликтов с помощью QMIX. Также мы предполагаем, что использование адаптивного составления задач для обучения агента (curriculum learning) также даст существенный прирост производительности для задач с большим количеством агентов



%\ack We would like to thank the referees for their comments, which helped improve this paper considerably

